Fixing a Broken ELBO

Recent work in unsupervised representation learning has focused on learning deep directed latent-variable models. Fitting these models by maximizing the marginal likelihood or evidence is typically intractable, thus a common approximation is to maximize the evidence lower bound (ELBO) instead. However, maximum likelihood training (whether exact or approximate) does not necessarily result in a good latent representation, as we demonstrate both theoretically and empirically. In particular, we derive variational lower and upper bounds on the mutual information between the input and the latent variable, and use these bounds to derive a rate-distortion curve that characterizes the tradeoff between compression and reconstruction accuracy. Using this framework, we demonstrate that there is a family of models with identical ELBO, but different quantitative and qualitative characteristics. Our framework also suggests a simple new method to ensure that latent variable models with powerful stochastic decoders do not ignore their latent code.

==> macros.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\H}{\operatorname{\sf H}}
\newcommand{\I}{\operatorname{\sf I}}
\newcommand{\E}{\operatorname{\sf E}}
\newcommand{\sm}{\softmax}
\newcommand{\lse}{\operatorname{\sf lse}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\chol}{\operatorname{chol}}
\newcommand{\subtril}{\operatorname{subtril}}
\newcommand{\iid}{\mbox{$\;\stackrel{\mbox{\tiny\rm iid}}{\sim}\;$}}
\def\tee{\textsf{\text{T}}\,}
\newtheorem{claim}{Claim}
\newtheorem{lemma}{Lemma}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}
\newcommand{\ba}{\begin{align*}}
\newcommand{\ea}{\end{align*}}
% \DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\onehot}{onehot}

\newcommand{\myvec}[1]{\mathbf{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\mytensor}[1]{\mathbf{\tilde{#1}}}

% Numbers
\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}

% Greek https://www.latex-tutorial.com/symbols/greek-alphabet/
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vvarepsilon}{\myvecsym{\varepsilon}}
\newcommand{\vzeta}{\myvecsym{\zeta}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
%\newcommand{\vEta}{\myvecsym{\Eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vmut}{\myvecsym{\tilde{\mu}}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
%\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vPi}{\myvecsym{\Pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vrho}{\myvecsym{\rho}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vthetat}{\myvecsym{\tilde{\theta}}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vSigmat}{\myvecsym{\tilde{\Sigma}}}
\newcommand{\vsigmoid}{\vsigma}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vxi}{\myvecsym{\xi}}


% Lower Roman (Vectors)
\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vBt}{\myvec{\tilde{B}}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
%\newcommand{\myvh}{\myvec{h}}
\newcommand{\vi}{\myvec{i}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\ttilde}{\tilde{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwt}{\myvec{\tilde{w}}}
\newcommand{\vWt}{\myvec{\tilde{W}}}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
\newcommand{\vxh}{\hat{\vx}}
\newcommand{\vxp}{\vx\myvec{'}}
\newcommand{\vxstar}{\vx^\myvec{\ast}}
\newcommand{\vxhstar}{\vxh^\myvec{\ast}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vxd}[1]{\vx_{:,#1}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyp}{\vy\myvec{'}}
\newcommand{\yh}{\hat{y}}
\newcommand{\vyh}{\hat{\vy}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}
\newcommand{\vzstar}{\vz^\myvec{\ast}}

% \newcommand{\vzt}{\myvec{\tilde{z}}}

% Upper Roman (Matrices)
\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vMt}{\myvec{\tilde{M}}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}
\newcommand{\vZt}{\myvec{\tilde{Z}}}
\newcommand{\vzt}{\myvec{\tilde{z}}}

% tensors
\newcommand{\tX}{\mytensor{X}}
\newcommand{\tY}{\mytensor{Y}}
\newcommand{\tZ}{\mytensor{Z}}
\newcommand{\tW}{\mytensor{W}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbS}{\mathbb{S}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\mymathcal}[1]{\pazocal{#1}}
\newcommand{\mymathcal}[1]{\mathcal{#1}}
%\usepackage{calrsfs}
%\DeclareMathAlphabet{\pazocal}{OMS}{zplm}{m}{n}
%http://tex.stackexchange.com/questions/69085/two-different-calligraphic-font-styles-in-math-mode

\newcommand{\calA}{\mymathcal{A}}
\newcommand{\calB}{\mymathcal{B}}
\newcommand{\calC}{\mymathcal{C}}
\newcommand{\calD}{{\mymathcal{D}}}
\newcommand{\calDx}{\calD_x}
\newcommand{\calE}{\mymathcal{E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{\mymathcal{F}}
\newcommand{\calG}{\mymathcal{G}}
\newcommand{\calH}{\mymathcal{H}}
\newcommand{\calHX}{{\calH}_X}
\newcommand{\calHy}{{\calH}_y}
\newcommand{\calI}{\mymathcal{I}}
\newcommand{\calK}{\mymathcal{K}}
\newcommand{\calM}{\mymathcal{M}}
\newcommand{\calN}{\mymathcal{N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{\mymathcal{NP}}
\newcommand{\calO}{\mymathcal{O}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{\mymathcal{L}}
\newcommand{\calP}{\mymathcal{P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{\mymathcal{Q}}
\newcommand{\calR}{\mymathcal{R}}
\newcommand{\calr}{\mymathcal{r}}
\newcommand{\calS}{\mymathcal{S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{\mymathcal{T}}
\newcommand{\calU}{\mymathcal{U}}
\newcommand{\calV}{\mymathcal{V}}
\newcommand{\calW}{\mymathcal{W}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{\mymathcal{X}}
\newcommand{\calY}{\mymathcal{Y}}
\newcommand{\calZ}{\mymathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%http://tex.stackexchange.com/questions/128625/how-to-put-smallsmile-or-smallfrown-on-top-of-a-letter/128626
 \newcommand{\adjustedaccent}[1]{%
   \mathchoice{}{}
     {\mbox{\raisebox{-.5ex}[0pt][0pt]{$\scriptstyle#1$}}}
     {\mbox{\raisebox{-.35ex}[0pt][0pt]{$\scriptscriptstyle#1$}}}
 }

\newcommand\smileacc[1]{\overset{\adjustedaccent{\smallsmile}}{#1}}
\newcommand\frownacc[1]{\overset{\adjustedaccent{\smallfrown}}{#1}}
%\newcommand\smileacc[1]{\overset{\smallsmile}{#1}}
%\newcommand\frownacc[1]{\overset{\smallfrown}{#1}}

%\newcommand{\prior}[1]{\breve{{#1}}}
\newcommand{\prior}[1]{\smileacc{#1}}
\newcommand{\post}[1]{\frownacc{#1}} % inverted breve
%\newcommand{\post}[1]{\stackrel{\smallfrown}{{#1}}} % inverted breve
%\newcommand{\post}[1]{\stackon{{#1}}{\smallfrown}} % inverted breve
%\newcommand{\post}[1]{\newtie{{#1}}} % inverted breve
%\newcommand{\post}[1]{\tilde{{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\betadist}{\mathrm{Beta}}
\newcommand{\Betadist}{\mathrm{Beta}}
\newcommand{\bernoulli}{\mathrm{Ber}}
\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Binom}{\mathrm{Bin}}
\newcommand{\BinoDist}{\mathrm{Bin}}
\newcommand{\NegBinom}{\mathrm{NegBinom}}
\newcommand{\binomdist}{\mathrm{Bin}}
\newcommand{\cauchy}{\mathrm{Cauchy}}
\newcommand{\DE}{\mathrm{DE}}
\newcommand{\DP}{\mathrm{DP}}
\newcommand{\Dir}{\mathrm{Dir}}
%\newcommand{\discrete}{\mathrm{Discrete}}
\newcommand{\discrete}{\mathrm{Cat}}
\newcommand{\cat}{\mathrm{Cat}}
\newcommand{\Cat}{\mathrm{Cat}}
\newcommand{\data}{\calD}
\newcommand{\Discrete}{\discrete}
\newcommand{\erlang}{\mathrm{Erlang}}
\newcommand{\expdist}{\mathrm{Expon}}
\newcommand{\expon}{\mathrm{Expon}}
\newcommand{\expfam}{\mathrm{Expfam}}
\newcommand{\Expfam}{\mathrm{Expfam}}
\newcommand{\gammadist}{\mathrm{Ga}}
\newcommand{\Ga}{\mathrm{Ga}}
\newcommand{\GP}{\mathrm{GP}}
\newcommand{\GEM}{\mathrm{GEM}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\gausscan}{\mathcal{N}_c}
\newcommand{\geom}{\mathrm{Geom}}
%\newcommand{\IG}{\mathrm{InvGam}}
\newcommand{\IG}{\mathrm{IG}}
\newcommand{\IGauss}{\mathrm{InvGauss}}
\newcommand{\invchi}{\chi^{-2}}
\newcommand{\IW}{\mathrm{IW}}
\newcommand{\Laplace}{\mathrm{Lap}}
\newcommand{\logisticdist}{\mathrm{Logistic}}
\newcommand{\Mu}{\mathrm{Mu}}
\newcommand{\Multi}{\mathrm{Mu}}
%\newcommand{\Multin}{\mathrm{Mun}}
%\newcommand{\Mun}{\mathrm{Mun}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mathrm{NIG}}
\newcommand{\GIG}{\mathrm{NIG}}
\newcommand{\NIW}{\mathrm{NIW}}
\newcommand{\GIW}{\mathrm{NIW}}
\newcommand{\GT}{{\mathrm{GT}}}
%\newcommand{\MVNIW}{\mathrm{MVNIW}}
\newcommand{\MVNIW}{\mathrm{NIW}}
\newcommand{\NW}{\mathrm{NWI}}
\newcommand{\NWI}{\mathrm{NWI}}
%\newcommand{\MVNIG}{\mathrm{MVNIG}}
\newcommand{\MVNIG}{\mathrm{NIG}}
\newcommand{\NGdist}{\mathrm{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mathrm{Poi}}
\newcommand{\RV}{RV}
\newcommand{\softmax}{\calS}
\newcommand{\Student}{\mathcal{T}}
\newcommand{\student}{\mathcal{T}}
\newcommand{\unif}{\mathrm{Unif}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\Wishart}{\mathrm{Wi}}
\newcommand{\Wi}{\mathrm{Wi}}

\newcommand{\fdec}{f_{\mathrm{dec}}}
\newcommand{\fenc}{f_{\mathrm{enc}}}
\newcommand{\fdisc}{f_{\mathrm{disc}}}
\newcommand{\fclass}{f_{\mathrm{class}}}
\newcommand{\vxhadv}{\vxh_{\mathrm{adv}}}
\newcommand{\Gtarg}{G_{\mathrm{targ}}}
\newcommand{\VAE}{\mathrm{VAE}}
\newcommand{\classifier}{\mathrm{classifier}}
\newcommand{\latent}{\mathrm{latent}}
\newcommand{\CA}{\mathrm{CA}}

\newcommand{\hmm}[1]{\ifnum\ifhmode\spacefactor\else2000\fi>1000 \uppercase{#1}\else#1\fi}

\newcommand{\ASuntargeted}{AS_{ignore-target}}
\newcommand{\AStargeted}{AS_{target}}
% \DeclareMathOperator{\Oracle}{Oracle}
\newcommand{\LX}{L_{\calX}}
\newcommand{\LY}{L_{\calY}}

\newcommand{\na}[1]{\textit{IR2-\ifnum0=#1Base-Deconv\else \ifnum1=#1Conv-FC\else \ifnum2=#1Conv-Deconv\else \ifnum3=#1Resize-Conv\else ERROR\fi\fi\fi\fi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\cbar}{\overline{c}}
\newcommand{\vcbar}{\overline{\vc}}
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vAbar}{\overline{\vA}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\wbar}{\overline{w}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Abar}{\overline{A}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}
\newcommand{\mubar}{\overline{\mu}}
\newcommand{\phibar}{\overline{\phi}}


